Uncertainty Quantification in Multiscale Modeling of Polymer Composite Materials Using Physically Recurrent Neural Networks

This study investigates whether Physically Recurrent Neural Networks (PRNNs), a recent surrogate model for heterogeneous materials, trained on a micromodel with fixed material parameters, can maintain accuracy for varying material properties without retraining, and propagate uncertainty in a multiscale framework. Unlike conventional RNNs, where parameter changes require training or explicit inclusion of material properties as extra input features, PRNNs embeds material models in their material layer that allow for modification of material parameters after training. When adjusting material properties dynamically according to the input during testing, PRNN shows high accuracy across a wide range of parameters. Therefore the surrogate can be applied to multiscale uncertainty quantification (UQ). Compared to the full-order simulations on an overly coarse mesh, the PRNN-driven model reduces simulation time by over 7000 times while accurately capturing highly nonlinear evolution of the probability density for the macroscopic response as a result of a given distribution for microscale material parameters. A PRNN-driven UQ is demonstrated on a more accurate finer mesh that would be computationally infeasible with the full-order model.

==> test.tex <==
The finite element model of the microstructure is shown in Figure \ref{fig:micro}, which consists of 25 periodically arranged fibers with diameter of $\SI{5}{\micro\metre}$ embedded in a matrix to result in a fiber volume fraction of 0.6. The matrix is modeled by a J2 plasticity model and a linear elastic model is used for the fibers. The geometry and mesh of the micromodel is kept constant in this paper. The material properties in \cite{MAIA2023115934} are used as reference in this work, which are: the Young's modulus of the matrix and the fiber ($E_m = 3,130 MPa$ and $E_f = 74,000 MPa$), Poisson's ratio of the matrix and the fiber ($\nu_m = 0.37$ and $\nu_f = 0.2$), and the yield strength of the matrix ($\sigma_y = 64.8 MPa$) with exponential hardening. 

\begin{figure}[!h]
\centering
\includegraphics[scale=2.]{micr.png}
\caption{\centering Full-order micromodel}
\label{fig:micro}
\end{figure}

The test data was generated by loading the micromodel in 10 predefined random directions for each parameter. 

$E_m = [200,10200,200]$
$n_m = [0.1,0.74,0.02]$ rerun w smaller timestep, some are missing
$plc = [49,112,3]$
$E_f = [40000,100000,1200]$
$n_f = [0.1,1.1,0.02]$

em x plc []

For one of the predefined directions, the resulting load-displacement curves are shown in Figures x-x for each parameter studied. It can be observed that varying the youngs modulus and poissons ratio of the fibers, and the poissons ratio of the matrix, there is no significant difference between the resulting curves. Therefore, with this slight variation, it is assumed that the pretrained PRNN wiht fixed parameters will be able to accurately predict for the varying parameters, therefore the study is continued with examining the effect of varying the youngs modulus and yield strength of the matrix.

\begin{figure}[htbp]
    \centering
    \begin{minipage}{\textwidth}
    \centering
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{testEmwg.pdf}
        \caption{youngs matrix}
        \label{em}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{testnmg.pdf}
        \caption{poissons matrix}
        \label{nm}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{testplcwg.pdf}
        \caption{yield strength}
        \label{plc}
    \end{subfigure}
    \end{minipage}
    \vskip\baselineskip
    \begin{minipage}{0.66\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{testEfg.pdf} 
        \caption{youngs fiber}
        \label{ef}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{testnfg.pdf}
        \caption{poissons fiber}
        \label{nf}
    \end{subfigure}
    \end{minipage}
    \caption{test curves}
    \label{fig:main}
\end{figure}

